Jointly optimal dereverberation and beamforming

We previously proposed an optimal (in the maximum likelihood sense) convolutional beamformer that can perform simultaneous denoising and dereverberation, and showed its superiority over the widely used cascade of a WPE dereverberation filter and a conventional MPDR beamformer. However, it has not been fully investigated which components in the convolutional beamformer yield such superiority. To this end, this paper presents a new derivation of the convolutional beamformer that allows us to factorize it into a WPE dereverberation filter, and a special type of a (non-convolutional) beamformer, referred to as a wMPDR beamformer, without loss of optimality. With experiments, we show that the superiority of the convolutional beamformer in fact comes from its wMPDR part.

==> tikz_header.tex <==
% Use TikZ to draw images
\usepackage{pgfplots} % Import der Plots aus Matlab
\newlength\fheight % Plots aus Matlab immer gleich gross
\newlength\fwidth % Plots aus Matlab immer gleich gross
\newlength{\figureheight} % Plots aus Matlab immer gleich gross
\newlength{\figurewidth} % Plots aus Matlab immer gleich gross
\usepackage{tikz}
\pgfplotsset{compat=1.9}

% Precompile TikZ pictures for speedup, this does not seem to work in Poolroom yet
\usetikzlibrary{external}
% \tikzexternalize % Activate, works only with pdflatex

\usetikzlibrary{arrows}
\usetikzlibrary{patterns}
\usetikzlibrary{backgrounds}
\usetikzlibrary{fit}
\usetikzlibrary{positioning}
\usetikzlibrary{shapes.geometric}
\usetikzlibrary{calc}
\usetikzlibrary{shapes.multipart}
\usetikzlibrary{shapes.misc}


\newlength{\baseunit}


